GlucoSynth: Generating Differentially-Private Synthetic Glucose Traces

We focus on the problem of generating high-quality, private synthetic glucose traces, a task generalizable to many other time series sources. Existing methods for time series data synthesis, such as those using Generative Adversarial Networks (GANs), are not able to capture the innate characteristics of glucose data and cannot provide any formal privacy guarantees without severely degrading the utility of the synthetic data. In this paper we present GlucoSynth, a novel privacy-preserving GAN framework to generate synthetic glucose traces. The core intuition behind our approach is to conserve relationships amongst motifs (glucose events) within the traces, in addition to temporal dynamics. Our framework incorporates differential privacy mechanisms to provide strong formal privacy guarantees. We provide a comprehensive evaluation on the real-world utility of the data using 1.2 million glucose traces; GlucoSynth outperforms all previous methods in its ability to generate high-quality synthetic glucose traces with strong privacy guarantees.

==> 6.related_work.tex <==


\section{Related Work}\label{sec:rel-work}

% \subsection{Previous Methods}
% A popular method to generate synthetic data is using Generative Adversarial Networks (GANs)~\cite{goodfellow2020generative}.
We overview related work in three lines of research: time series, conditional time series, and time series methods that employ differential privacy. Table~\ref{table:prev-methods} summarizes 
% the characteristics of 
previous time series synthesis methods.
We note that there have been exciting developments %in new approaches 
for adjacent research tasks (data augmentation, forecasting) such as diffusion models~\cite{alcaraz2022diffusion}, but there are not yet any publicly available models specifically for the generation of complete synthetic time series datasets. 
% but there are not yet any publicly available models specifically for this problem of the generation of complete time series synthetic datasets. 
As such, we focus the scope of our comparison on the current state-of-the-art methods for synthetic time series which all build upon Generative Adversarial Networks (GANs)~\cite{goodfellow2020generative} and transformation-based approaches~\cite{dinh2016density}. In particular TimeGAN~\cite{yoon2019time}, 
RGAN~\cite{esteban2017real} and dpGAN~\cite{frigerio2019differentially}
are most similar to ours and used as benchmarks in the evaluation in Section~\ref{sec-eval}.



%GANs + time series
\textbf{Time Series.} 
% There have been promising models to generate synthetic time series across a variety of domains such as financial data~\cite{dogariu2022generation}, cyber-physical systems (e.g., smart homes~\cite{razghandi2022variational}), and medical signals~\cite{hazra2020synsiggan}. 
\citet{brophy2021generative} provides a survey of GANs for time series synthesis.  
TimeGan~\cite{yoon2019time} is a popular benchmark that jointly learns an embedding space using supervised and adversarial objectives in order to capture the temporal dynamics amongst traces. TTS-GAN~\cite{ttsgan2022}, trains a GAN model that uses a transformer encoding architecture in order to best preserve temporal dynamics. Transformation-based approaches have also had success for time series data. Real-valued non-volume preserving transformations (NVP)~\cite{dinh2016density} model the underlying distribution of the real data using generative probabilistic modeling and use this model to output a set of synthetic data. Similarly, Fourier Flows (FF)~\cite{alaa2020generative} transform input traces into the frequency domain and output a set of synthetic data from the learned spectral representation of the original data. Methods that only focus on learning the temporal or distributional dynamics in time series are not sufficient for generating \textit{realistic} synthetic glucose traces due to the lack of temporal dependence within sequences of glucose motifs. 
% In fact, as shown in the evaluation section, autoregressive models learn to generate valid local patterns (short sequential series of glucose values within short time chunks) in the synthetic data but fail to construct synthetic traces with realistic (physiologically possible) overall sequences of motifs.
% Methods that only focus on conserving the temporal dependence amongst time series %(e.g., autoregressive models) 
% may not be sufficient to learn the relationships amongst sequences of motifs in glucose traces due to their lack of temporal dependence. 
% In fact, we show in the evaluation section that models that do \textit{only} rely on autoregressive architectures do not work well for generating synthetic data for glucose data.

% Previous time-series specific methods rely on seasonality trends, parallel trends, pattern-based timeseries, anomaly-based traces, autocorrelation(s) between multivariate time series (i.e., multiple features), or supervised methods (e.g., using labels). However, Glucose (and many other time series) traces do not have these common phenomenon: 
% Do not have strong, uniform/consistent seasonality
% Limited recurring patterns 
% No extra features or labels to guide learning


%conditional time
\textbf{Conditional Time Series.} Many works have developed time series models that supplement their training %through the use of additional information such as 
using extra features or conditional data. 
\citet{esteban2017real} develops two GAN models (RGAN/RCGAN) with RNN architectures, conditioned on 
% additional 
auxiliary information provided at each timestep during training. SigCWGAN~\cite{ni2020conditional} uses a mathematical conditional metric ($Sig-W_1$) characterizing the signature of a path to capture temporal dependence of joint probability distributions in long time series data. However, our glucose traces do not have any additional information available so these methods cannot be used\footnote{There is a caveat here that RGAN does not use auxillary information, hence why we compare with it in our benchmarks.}.
% e.g., any information about eating or other patient behaviors, 
%and therefore cannot use these methods. 


% gan + privacy general
\textbf{Differentially-Private GANs.} 
To protect sensitive data, several GAN architectures (DP GANs) have been designed to incorporate privacy-preserving noise needed to satisfy differential privacy guarantees~\cite{xie2018differentially}. 
% Since many datasets contain sensitive artifacts, especially in medical contexts, and GANs themselves do not formally preserve privacy (and in fact have been shown to be vulnerable to privacy attacks~\cite{che2016mode, hayes2017logan}), several GAN architectures (DP GANs) have been designed to incorporate privacy-preserving noise needed to satisfy differential privacy guarantees~\cite{xie2018differentially}. 
Although DP GANs such as 
% \dnote{really mean i.e. here, not just one example? I tried to reword the sentence above to be more clear that we are calling any method that involves a GAN and some mechanism to ensure DP a "DP GAN", but if you mean something more specific by this should be clear} 
PateGAN~\cite{jordon2018pate} have had great success for other data types and learning tasks (e.g., tabular data, supervised classification tasks), results have been less satisfactory 
% more of a mixed bag  
in DP GANs developed for time series.
% in terms of time series GAN models that include \textit{privacy}, results have been more of a mixed bag. 
% Of those that include strong privacy guarantees, many have very high utility-privacy trade offs. 



RGAN/RCGAN~\cite{esteban2017real} also includes a DP implementation, %for some tasks, 
but the authors find large gaps in performance between the nonprivate and private models. 
% For instance, the private model produces traces that are noticeably less realistic than those not trained with privacy. \dnote{isn't this just restating the previous sentence? in what way are the traces produced with privacy less good?}
% and those that include privacy, as well as visual traces that are noticeably (visually) less realistic than those not trained with privacy; produces less realistic sequences. 
\citet{frigerio2019differentially} extends a simple DP GAN architecture (denoted dpGAN) to 
to time-series data. The synthetic data from their private model conserves the distribution of the real data but loses some of the variability (diversity) from the original samples. RDP-CGAN~\cite{torfi2022differentially} develops a convolutional GAN architecture that uses R\'{e}nyi differential privacy specifically for medical data. Across different datasets, they find that reasonable privacy budgets result in major drops in the performance of the synthetic data. Finally, DoppelGANger~\cite{lin2020using} develops a temporal GAN framework for time series with metadata and perform an in-depth privacy evaluation. 
% with respect to protecting business secrets contained in the data and protecting individual user privacy. 
Notably, they find that providing strong theoretical DP guarantees results in destroying the fidelity of the synthetic data, beyond anything feasible for use in real-world scenarios. 
Each of these methods touches on the innate challenge of generating DP synthetic time series due to very high tradeoffs between utility and privacy.
\dnote{can we add a sentence that says how we overcome this challenge and do better?}

% Each of these methods touches on the innate challenge between utility and privacy for time series synthetic data. In particular, many have large tradeoffs that come at a high cost to the usability and fidelity of the synthetic data.
% many have very high utility-privacy trade offs. 










